Steering Fields: Adaptive Vector Fields for Safe Image Generation and Beyond

As state-of-the-art text-to-image flow models achieve near-photorealistic quality, controlling their outputs, e.g., suppressing harmful content while promoting benign alternatives, has become a central challenge. The current steering paradigm consists of adding a global steering vector to selected activations. While functional, a fixed and example-agnostic vector applied uniformly along the entire trajectory cannot adapt to the changing state of the generation and often causes unintended global changes. We introduce Steering Fields, a generalization of steering vectors that adaptively re-estimates the steering direction at each step of the generative process. Steering Fields operate on the noisy states of flow models, expose a continuous trade-off between steering strength and content preservation, and are compositional, enabling the simultaneous induction and inhibition of concepts, setting a new state of the art on safety steering benchmarks. Despite using no explicit spatial masks or object priors, the trajectory-adaptive estimation naturally preserves local structure, in a manner reminiscent of image editing. In fact, Steering Fields can serve as a structure-preserving image-editing technique that achieves state-of-the-art semantic fidelity (CLIP, VQAScore), while remaining model-agnostic and inversion-free.

==> figures/steering_density_3baselines.tex <==
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/density_vqascore_vs_nudenet_3clusters.png}
%         % \caption{FLUX}
%         \label{fig:density_flux}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/density_vqascore_vs_nudenet_3clusters_sd35.png}
%         % \caption{SD3.5}
%         \label{fig:density_sd35}
%     \end{subfigure}
%     \caption{\SF{add ESD and UCE} Trade-off between NSFW suppression and semantic fidelity on Ring-a-Bell. Each contour shows the joint distribution of NudeNet score (lower is safer) and VQAScore on COCO-1k (higher is better). Steering Fields (blue, solid) achieves stronger safety than competing methods while preserving semantic quality close to the vanilla baseline (gray, dashed).}
%     \label{fig:density}
% \end{figure}


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/density_vqascore_vs_nudenet_3clusters_sd35.png}
%     \caption{Trade-off between NSFW suppression and semantic fidelity on Ring-a-Bell for SD as base model. Each contour shows the joint distribution of NudeNet score (lower is safer) and VQAScore on COCO-1k (higher is better). Steering Fields (blue, solid) achieves stronger safety than competing methods while preserving semantic quality close to the vanilla baseline (gray, dashed).}
%     \label{fig:density_sd}
% \end{figure}

\begin{figure}[h!]
    \centering

    \begin{subfigure}[t]{0.50\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/density_vqascore_vs_nudenet_3clusters.png}
        \caption{VQAScore vs. Nudenet on FLUX1}
        \label{fig:density_flux}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/density_vqascore_vs_nudenet_3clusters_sd35.png}
        \caption{VQAScore vs. Nudenet on SD3.5}
        \label{fig:density_sd35}
    \end{subfigure}

    \caption{Trade-off between NSFW suppression and semantic fidelity on Ring-a-Bell, for both FLUX1 (left) and SD3.5 (right). Each contour shows the joint distribution of NudeNet score (lower is safer) and VQAScore on COCO-1k (higher is better). Steering Fields (blue, solid) achieves stronger safety than competing methods while preserving semantic quality close to the vanilla baseline (gray, dashed).}
    \label{fig:densities_flux_sd}
\end{figure}

==> figures/steering_density_5baselines.tex <==
%%%% In the original submission:
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[t]{0.42\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{qual/safety.pdf}
%         \label{fig:safety_qual}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.55\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/density_vqascore_vs_nudenet_3clusters.png}
%         \label{fig:density}
%     \end{subfigure}
%     \vspace{-0.3cm}
%     \caption{\textbf{(left) Qualitative results} steering away from nudity across samples from the P4D and Ring-a-Bell dataset, comparing Baseline, EraseAnything, and Steering Fields (ours). \textbf{(right) Trade-off between NSFW suppression and semantic fidelity.} Each contour shows the joint distribution of NudeNet score on Ring-a-Bell (lower is safer) and VQAScore on COCO-1k (higher is better). Steering Fields (\textcolor{blue}{solid}) achieves stronger safety than competitors while preserving semantic quality close to the baseline (\textcolor{gray}{dashed}). \SF{Do we need this figure now? Maybe not}}
%     \vspace{-0.5cm}
%     \label{fig:safety_combined}
% \end{figure}

\SF{here we used to have the other figure: it's commented in the latex docs}

==> tables/editing_change_clip_metrics.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|cccc}
\hline
\textbf{Method} & \textbf{CLIP-txt $\uparrow$} & \textbf{CLIP-img $\uparrow$} & \textbf{CLIP-dir $\uparrow$} & \textbf{VQAScore $\uparrow$} \\
\hline
Flux Img2Img & -- \std{--} & -- \std{--} & -- \std{--} & -- \std{--} \\
StableFlow   & -- \std{--} & -- \std{--} & -- \std{--} & -- \std{--} \\
FlowEdit     & -- \std{--} & -- \std{--} & -- \std{--} & -- \std{--} \\
Ours         & -- \std{--} & -- \std{-} & -- \std{--} & -- \std{--} \\
\hline
\end{tabular}
\caption{Semantic metrics, overall on 64 seeds.}
\end{table}

==> tables/editing_change_pixel_metrics.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|ccccc}
\hline
\textbf{Method} & \textbf{PSNR $\uparrow$} & \textbf{LPIPS $\downarrow$} & \textbf{MSE $\downarrow$} & \textbf{SSIM $\uparrow$} & \textbf{FID $\downarrow$} \\
\hline
Flux Img2Img & 17.26 \std{.0460} & 0.49 \std{.0020} & 0.021 \std{.0002} & 0.490 \std{.0029} & 186.36 \std{1.01} \\
StableFlow   & 19.45 \std{.0008} & 0.20 \std{.0001} & 0.015 \std{.0001} & 0.801 \std{.0001} & 114.03 \std{0.07} \\
FlowEdit     & 17.56 \std{.0037} & 0.33 \std{.0005} & 0.021 \std{.0002} & 0.699 \std{.0012} & 170.05 \std{0.81} \\
Ours         & 16.07 \std{.0430} & 0.52 \std{.0016} & 0.027 \std{.0003} & 0.477 \std{.0023} & 191.42 \std{0.86} \\
\hline
\end{tabular}
\caption{Pixel-level metrics, overall on 64 seeds.}
\end{table}

==> tables/editing_overall_pixel_metrics.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|ccccc}
\hline
\textbf{Method} & \textbf{PSNR $\uparrow$} & \textbf{LPIPS $\downarrow$} & \textbf{MSE $\downarrow$} & \textbf{SSIM $\uparrow$} & \textbf{FID $\downarrow$} \\
\hline
Flux Img2Img & 17.48 \std{.1677} & 0.464 \std{.0017} & 0.021 \std{.0009} & 0.503 \std{.0134} & 169.13 \std{0.68} \\
StableFlow   & \textbf{19.87} \std{.5465} & \textbf{0.183} \std{.0001} & \textbf{0.014} \std{.0017} & \textbf{0.810} \std{.0084} & \textbf{96.13} \std{0.07} \\
FlowEdit     & 18.26 \std{.3445} & 0.295 \std{.0006} & 0.018 \std{.0014} & 0.725 \std{.0119} & 137.50 \std{0.51} \\
Ours         & 16.27 \std{.1542} & 0.492 \std{.0013} & 0.027 \std{.0011} & 0.490 \std{.0144} & 169.30 \std{0.47} \\
\hline
\end{tabular}
\caption{Pixel-level metrics, overall on 64 seeds.}
\end{table}
